Recurrent Drafter for Fast Speculative Decoding in Large Language Models

We present Recurrent Drafter (ReDrafter), an advanced speculative decoding approach that achieves state-of-the-art speedup for large language models (LLMs) inference. The performance gains are driven by three key aspects: (1) leveraging a recurrent neural network (RNN) as the draft model conditioning on LLM's hidden states, (2) applying a dynamic tree attention algorithm over beam search results to eliminate duplicated prefixes in candidate sequences, and (3) training through knowledge distillation from the LLM. ReDrafter accelerates Vicuna inference in MT-Bench by up to 2.8x with a PyTorch implementation on Nvidia H100 GPUs. To demonstrate its practicality in real environments, we also validated its effectiveness for on-device applications by implementing the approach in MLX and benchmarking performance on Metal GPUs in Apple Silicon chips, achieving up to 2.3x speedup.

==> ICLR2025_submission/figures/explain_dynamic_tree_attention.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\textwidth]{ICLR2025_submission/figures/tree_attention_implementation.pdf} 
    %\vspace{-0.3in}
    \caption{An illustration of the different components for building the dynamic tree attention for batch size equals to 1. (Extending to batch size larger than 1 is straighforward.) In this example, the beam size is $3$, with each candidate sequence containing $4$ tokens. (a) The beam search result.  (b) The total token count is reduced from $3\times 4=12$ to $9$ by compressing shared prefixes in the beam search result. (c) A tensor-based, GPU-friendly algorithm is used to detect repeating prefixes within each beam (illustrated as gray boxes). (d) The tensor-based approach also extends to the encoding of child-parent relationships in the tree attention. The attention masks can be applied in a similar way.}
    \label{fig:explain-dynamic-tree-attention}
\end{figure}

==> ICLR2025_submission/figures/narrow_beam.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{ICLR2025_submission/figures/narrow_beam.pdf}
   \caption{(a) We incorporate beam search during training to optimize its inference performance. During training, we identify the first rejected token in each beam path and focus on optimizing those tokens. (b) narrow beam.}
   \label{fig:narrow_beam}
\end{figure}

==> ICLR2025_submission/tables/beam_search_tree_attention.tex <==
\begin{table}[h]
\centering
\caption{TFLOPs and compression ratio \(\rho\) for ReDrafter Vicuna 7B with and without tree attention (TA) when batch size equals to 1.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
% & \multicolumn{10}{c}{Beam Width (BW)} \\
% \cmidrule(l){2-11}
\multirow{2}{*}{Method} & \multicolumn{2}{c}{BW=1} & \multicolumn{2}{c}{BW=2} & \multicolumn{2}{c}{BW=4} & \multicolumn{2}{c}{BW=16} & \multicolumn{2}{c}{BW=64} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11}
& TFLOPs & \(\rho\) & TFLOPs & \(\rho\) & TFLOPs & \(\rho\) & TFLOPs & \(\rho\) & TFLOPs & \(\rho\)\\
\midrule
 w/o TA & \tbd{207.0} & 1.00 & \tbd{215.0} & 1.00 & \tbd{221.0} & 1.00 & \tbd{235.0} & 1.00 & \tbd{242.0} & 1.00\\
 with TA & \tbd{207.0} & \tbd{2.59} & \tbd{225.0} & \tbd{2.78} & \tbd{235.0} & \tbd{2.85} & \tbd{247.0} & \tbd{3.03} & \tbd{259.0} & \tbd{3.15} \\
\bottomrule
\end{tabular}
}
\label{table:beam_search_tree_attention}
\end{table}

==> ICLR2025_submission/tables/pytorch_benchmark_alpaca.tex <==
\begin{table}[t]
\centering
\caption{Speedup and \(\tau\) for Medusa, EAGLE, and ReDrafter on AlpacaEval.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
\multicolumn{12}{c}{AlpacaEval,~temperature=0 \cmnt{7B 33.43, 13B 26.89, 33B 16.61}} \\
\midrule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Helpful} & \multicolumn{2}{c}{Koala} & \multicolumn{2}{c}{OASST} & \multicolumn{2}{c}{Self-instruct} & \multicolumn{2}{c}{Vicuna Test} & \multicolumn{2}{c}{Average} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14}
 & & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) \\
\midrule
\multirow{3}{*}{V 7B}
 & Medusa & 2.12x\cmnt{70.99} & 2.34 & 2.22x\cmnt{74.48} & 2.43 & 2.24x\cmnt{75.21} & 2.45 & 2.12x\cmnt{71.18} & 2.36 & 2.26x\cmnt{75.87} & 2.50 & 2.19x & 2.42 \\
 & EAGLE & 2.32x\cmnt{77.65} & 3.42 & 2.46x\cmnt{82.40} & 3.64 & 2.46x\cmnt{82.34} & 3.67 & 2.47x\cmnt{82.77} & 3.71 & 2.44x\cmnt{81.82} & 3.63  & 2.43x & 3.61 \\
 & ReDrafter & \bf{2.52x} & \bf{3.93} & \bf{2.72x} & \bf{4.10} & \bf{2.74x} & \bf{4.05} & \bf{2.61x} & \bf{3.89} & \bf{2.85x} & \bf{4.35} & \bf{2.69x} & \bf{4.06} \\
\midrule
\multirow{3}{*}{V 13B}
 & Medusa & 2.16x\cmnt{58.10} & 2.40 & 2.30x\cmnt{61.90} & 2.46 & 2.29x\cmnt{61.57} & 2.43 & 2.23x\cmnt{60.10} & 2.45 & 2.30x\cmnt{61.91} & 2.53 & 2.26x & 2.45 \\
 & EAGLE & 2.38x\cmnt{64.14} & 3.49 & 2.48x\cmnt{66.74} & 3.64 & 2.48x\cmnt{66.73} & 3.62 & 2.58x\cmnt{69.45} & 3.72 & 2.53x\cmnt{68.14} & 3.62 & 2.49x & 3.62\\
 & ReDrafter & \bf{2.66x} & \bf{3.89} & \bf{2.97x} & \bf{4.19} & \bf{2.68x} & \bf{3.81} & \bf{2.69x} & \bf{3.91} & \bf{2.91x} & \bf{4.33} &\bf{2.78x} & \bf{4.02}\\
\midrule
\multirow{3}{*}{V 33B}
 & Medusa & 2.30x\cmnt{38.30} & 2.26 & 2.30x\cmnt{38.33} & 2.29 & 2.32x\cmnt{38.62} & 2.33 & 2.29x\cmnt{38.12} & 2.31 & 2.35x\cmnt{39.19} & 2.35 & 2.31x & 2.31 \\
 & EAGLE & \bf{2.46x}\cmnt{40.90} & 3.11 & \bf{2.62x}\cmnt{43.61} & 3.33 & \bf{2.60x}\cmnt{43.35} & 3.32 & \bf{2.63x}\cmnt{43.84} & 3.36 & \bf{2.64x}\cmnt{43.98} & 3.32 & \bf{2.59x} & 3.29 \\
 & ReDrafter & {2.32x} & \bf{3.47} & {2.45x} & \bf{3.63} & {2.43x} & \bf{3.59} & {2.35x} & \bf{3.49} & {2.61x} & \bf{3.85} & 2.43x & \bf{3.61} \\
\midrule
\multicolumn{12}{c}{AlpacaEval,~temperature=1 \cmnt{7B 32.14, 13B 26.88, 33B 15.88}} \\
\midrule
\multirow{3}{*}{V 7B}
 & Medusa & 2.20x\cmnt{70.98} & 2.34 & 2.26x\cmnt{72.65} & 2.43 & 2.26x\cmnt{72.77} & 2.45 & 2.24x\cmnt{72.04} & 2.40 & 2.35x\cmnt{75.65} & 2.47 & 2.26x & 2.42 \\
 & EAGLE & 2.09x\cmnt{67.47} & 3.13 & 2.22x\cmnt{71.44} & 3.32 & 2.18x\cmnt{70.09} & 3.26 & 2.22x\cmnt{71.36} & 3.32 & 2.31x\cmnt{74.37} & 3.41 & 2.20x & 3.29 \\
 & ReDrafter & \bf{3.41x} & \bf{5.17} & \bf{3.63x} & \bf{5.38} & \bf{3.47x} & \bf{5.29} & \bf{3.41x} & \bf{5.22} & \bf{3.72x} & \bf{5.50} & \bf{3.53x} & \bf{5.31} \\
\midrule
\multirow{3}{*}{V 13B}
 & Medusa & 2.18x\cmnt{58.60} & 2.42 & 2.24x\cmnt{60.45} & 2.50 & 2.26x\cmnt{60.76} & 2.52 & 2.25x\cmnt{60.67} & 2.49 & 2.27x\cmnt{61.25} & 2.58 & 2.24x & 2.50 \\
 & EAGLE & 2.07x\cmnt{55.79} & 3.16 & 2.22x\cmnt{59.74} & 3.43 & 2.10x\cmnt{56.65} & 3.28 & 2.15x\cmnt{57.89} & 3.37 & 2.26x\cmnt{60.94} & 3.44 & 2.16x & 3.34 \\
 & ReDrafter & \bf{3.35x} & \bf{5.03} & \bf{3.59x} & \bf{5.27} & \bf{3.48x} & \bf{5.21} & \bf{3.41x} & \bf{5.13} & \bf{3.69x} & \bf{5.44} & \bf{3.50x} & \bf{5.22}\\
\midrule
\multirow{3}{*}{V 33B}
 & Medusa & 2.38x\cmnt{37.92} & 2.28 & 2.45x\cmnt{38.91} & 2.35 & 2.41x\cmnt{38.35} & 2.34 & 2.45x\cmnt{39.03} & 2.36 & 2.45x\cmnt{39.00} & 2.38 & 2.43x & 2.34 \\
 & EAGLE & 2.24x\cmnt{35.72} & 2.98 & 2.43x\cmnt{38.70} & 3.16 & 2.38x\cmnt{37.85} & 3.10 & 2.42x\cmnt{38.54} & 3.19 & 2.58x\cmnt{41.01} & 3.36 & 2.41x & 3.16 \\
 & ReDrafter & \bf{3.14x} & \bf{4.48} & \bf{3.33x} & \bf{4.78} & \bf{3.29x} & \bf{4.71} & \bf{3.34x} & \bf{4.71} & \bf{3.48x} & \bf{4.89} & \bf{3.32x} & \bf{4.71} \\
\bottomrule
\end{tabular}
}
\label{table:pytorch_benchmark_alpaca}
\end{table}

==> ICLR2025_submission/tables/pytorch_benchmark_mt_bench.tex <==
\begin{table}[t]
\centering
\caption{Speedup and \(\tau\) for Medusa, EAGLE, and ReDrafter on MT-Bench.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccccccccccccccc@{}}
\toprule
\multicolumn{18}{c}{MT-bench,~temperature=0 \cmnt{7B 33.43, 13B 26.89, 33B 16.61}} \\
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Writing} & \multicolumn{2}{c}{Roleplay} & \multicolumn{2}{c}{Reasoning} & \multicolumn{2}{c}{Math} & \multicolumn{2}{c}{Coding} & \multicolumn{2}{c}{Extraction} & \multicolumn{2}{c}{Stem} & \multicolumn{2}{c}{Humanities} & \multicolumn{2}{c}{Average} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14} \cmidrule(l){15-16} \cmidrule(l){17-18} \cmidrule(l){19-20} \cmidrule(l){21-22}
 & & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) \\
\midrule
\multirow{3}{*}{V 7B}
 & Medusa & 2.27x\cmnt{76.11} & 2.41 & 2.26x\cmnt{75.69} & 2.41 & 2.27x\cmnt{76.03} & 2.47 & 2.57x\cmnt{85.98} & 2.75 & 2.71x\cmnt{90.66} & 2.86 & 2.55x\cmnt{85.35} & 2.74 & 2.34x\cmnt{78.49} & 2.48 & 2.17x\cmnt{72.67} & 2.29 & 2.39x & 2.55 \\
 & EAGLE & 2.47x\cmnt{82.68} & 3.56 & 2.61x\cmnt{87.54} & 3.83 & 2.54x\cmnt{84.98} & 3.81 & 2.89x\cmnt{96.70} & 4.24 & 3.11x\cmnt{104.30} & 4.58 & \bf{2.91x}\cmnt{97.32} & \bf{4.39} & 2.54x\cmnt{85.03} & 3.71 & 2.45x\cmnt{82.17} & 3.52 & 2.69x & 3.96 \\
 & ReDrafter & \bf{2.77x} & \bf{4.18} & \bf{2.91x} & \bf{4.50} & \bf{2.59x} & \bf{3.85} & \bf{2.96x} & \bf{4.34} & \bf{3.19x} & \bf{4.86} & {2.62x} & {3.93} & \bf{2.80x} & \bf{4.28} & \bf{2.52x} & \bf{3.69} & \bf{2.80x} & \bf{4.20}\\
\midrule
\multirow{3}{*}{V 13B}
 & Medusa & 2.27x\cmnt{61.10} & 2.46 & 2.28x\cmnt{61.37} & 2.48 & 2.21x\cmnt{59.46} & 2.46 & 2.66x\cmnt{71.71} & 2.89 & 2.75x\cmnt{73.97} & 2.97 & 2.43x\cmnt{65.45} & 2.66 & 2.36x\cmnt{63.48} & 2.54 & 2.23x\cmnt{60.02} & 2.39 & 2.40x & 2.61 \\
 & EAGLE & 2.59x\cmnt{69.82} & 3.74 & 2.41x\cmnt{64.92} & 3.48 & 2.51x\cmnt{67.64} & 3.80 & 3.08x\cmnt{82.99} & 4.49 & 3.07x\cmnt{82.79} & 4.43 & \bf{3.08x}\cmnt{82.88} & \bf{4.59} & 2.64x\cmnt{71.15} & 3.81 & 2.53x\cmnt{68.25} & 3.65 & 2.74x & 4.00 \\
 & ReDrafter & \bf{2.70x} & \bf{4.00} & \bf{2.80x} & \bf{4.22} & \bf{2.60x} & \bf{3.87} & \bf{3.11x} & \bf{4.61} & \bf{3.21x} & \bf{4.88} & {2.52x} & {3.91} & \bf{2.74x} & \bf{4.28} & \bf{2.69x} & \bf{3.92} & \bf{2.80x} &\bf{4.21} \\
\midrule
\multirow{3}{*}{V 33B}
 & Medusa & 2.24x\cmnt{37.37} & 2.24 & 2.33x\cmnt{38.86} & 2.32 & 2.44x\cmnt{40.60} & 2.48 & 2.83x\cmnt{47.15} & 2.82 & 2.90x\cmnt{48.20} & 2.94 & 2.71x\cmnt{45.09} & 2.85 & 2.40x\cmnt{40.01} & 2.40 & 2.25x\cmnt{37.43} & 2.22 & 2.51x & 2.53\\
 & EAGLE & 2.47x\cmnt{41.15} & 3.23 & 2.42x\cmnt{40.36} & 3.17 & \bf{2.68x}\cmnt{44.54} & 3.63 & \bf{3.26x}\cmnt{54.24} & 4.30 & \bf{3.36x}\cmnt{55.87} & 4.41 & \bf{3.12x}\cmnt{51.90} & \bf{4.32} & \bf{2.61x}\cmnt{43.49} & 3.41 & \bf{2.47x}\cmnt{41.06} & 3.21 & \bf{2.80x} & 3.71 \\
 & ReDrafter & \bf{2.50x} & \bf{3.63} & \bf{2.47x} & \bf{3.64} & {2.47x} & \bf{3.73} & {2.72x} & \bf{4.32} & {3.25x} & \bf{4.49} & {2.62x} & {3.95} & {2.55x} & \bf{3.79} & {2.26x} & \bf{3.43} & {2.61x} & \bf{3.87} \\
\midrule
\multicolumn{18}{c}{MT-bench,~temperature=1 \cmnt{7B 32.14, 13B 26.88, 33B 15.88}} \\
\toprule
\multirow{3}{*}{V 7B}
 & Medusa & 2.09x\cmnt{67.48} & 2.28 & 2.24x\cmnt{72.24} & 2.46 & 2.23x\cmnt{71.78} & 2.52 & 2.52x\cmnt{81.18} & 2.77 & 2.57x\cmnt{82.71} & 2.78 & 2.45x\cmnt{78.83} & 2.70 & 2.31x\cmnt{74.51} & 2.52 & 2.21x\cmnt{71.13} & 2.39 & 2.33x & 2.55 \\
 & EAGLE & 2.21x\cmnt{69.39} & 3.23 & 2.12x\cmnt{68.27} & 3.20 & 2.17x\cmnt{69.95} & 3.50 & 2.50x\cmnt{80.46} & 3.83 & 2.67x\cmnt{85.85} & 4.00 & 2.46x\cmnt{79.31} & 3.79 & 2.21x\cmnt{71.30} & 3.32 & 2.14x\cmnt{69.08} & 3.20 & 2.31x & 3.51 \\
 & ReDrafter & \bf{3.58x} & \bf{5.52} & \bf{3.59x} & \bf{5.54} & \bf{3.47x} & \bf{5.29} & \bf{3.63x} & \bf{5.43} & \bf{3.75x} & \bf{5.57} & \bf{3.16x} & \bf{4.85} & \bf{3.32x} & \bf{5.00} & \bf{3.49x} & \bf{5.27} & \bf{3.50x} & \bf{5.31} \\
\midrule
\multirow{3}{*}{V 13B}
 & Medusa & 2.22x\cmnt{59.90} & 2.47 & 2.22x\cmnt{59.90} & 2.47 & 2.23x\cmnt{59.98} & 2.53 & 2.60x\cmnt{69.98} & 2.91 & 2.64x\cmnt{71.05} & 2.92 & 2.40x\cmnt{64.67} & 2.69 & 2.35x\cmnt{63.30} & 2.54 & 2.21x\cmnt{59.45} & 2.38  & 2.36x & 2.61 \\`
 & EAGLE & 1.98x\cmnt{53.24} & 3.05 & 2.11x\cmnt{56.86} & 3.27 & 2.22x\cmnt{59.70} & 3.57 & 2.45x\cmnt{65.99} & 3.83 & 2.58x\cmnt{69.54} & 3.99 & 2.40x\cmnt{64.78} & 3.83 & 2.28x\cmnt{61.43} & 3.54 & 2.12x\cmnt{57.24} & 3.30 & 2.27x & 3.55 \\
 & ReDrafter & \bf{3.46x} & \bf{5.44} 
            & \bf{3.66x} & \bf{5.45} 
            & \bf{3.25x} & \bf{5.13} 
            & \bf{3.56x} & \bf{5.13} 
            & \bf{3.70x} & \bf{5.56} 
            & \bf{3.29x} & \bf{5.01} 
            & \bf{3.69x} & \bf{5.40} 
            & \bf{3.46x} & \bf{5.17} 
            & \bf{3.51x} & \bf{5.29}\\
\midrule
\multirow{3}{*}{V 33B}
 & Medusa & 2.28x\cmnt{36.25} & 2.19 & 2.50x\cmnt{39.74} & 2.37 & 2.55x\cmnt{40.51} & 2.46 & 2.90x\cmnt{46.21} & 2.75 & 3.03x\cmnt{48.21} & 2.97 & 2.72x\cmnt{43.31} & 2.79 & 2.46x\cmnt{39.14} & 2.40 & 2.28x\cmnt{36.34} & 2.23 & 2.59x & 2.52 \\
 & EAGLE & 2.22x\cmnt{35.33} & 2.93 & 2.38x\cmnt{37.92} & 3.14 & 2.57x\cmnt{40.93} & 3.47 & 2.98x\cmnt{47.43} & 3.89 & 3.18x\cmnt{50.64} & 4.14 & 2.84x\cmnt{45.16} & 3.91 & 2.45x\cmnt{38.98} & 3.18 & 2.41x\cmnt{38.37} & 3.14 & 2.63x & 3.48\\
 & ReDrafter & \bf{3.24x} & \bf{4.69} 
            & \bf{3.39x} & \bf{4.95} 
            & \bf{3.12x} & \bf{4.42} 
            & \bf{3.37x} & \bf{4.83} 
            & \bf{3.58x} & \bf{5.05} 
            & \bf{2.94x} & \bf{4.34} 
            & \bf{3.35x} & \bf{4.75} 
            & \bf{3.13x} & \bf{4.52} 
            & \bf{3.27x} & \bf{4.69}\\
\bottomrule
\end{tabular}
}
\label{table:pytorch_benchmark_mt_bench}
\end{table}

% TODO add a highlight to rows of ReDrafter
% TODO consider another presentation to distinguash from Eagle, or Change the table to bar plots? Or Transpose?


==> ICLR2025_submission/tables/pytorch_benchmark_t0.tex <==
\begin{table}[t]
\centering
\caption{Comparison of Speedup and \(\tau\) for Different Methods on Various Benchmarks (t=0). \aonan{Need to mention drafter size.}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
 & & \multicolumn{12}{c}{Benchmark} \\
\cmidrule(l){3-14}
Model & Method & \multicolumn{2}{c}{MT-bench} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{Alpaca} & \multicolumn{2}{c}{CNN/DM} & \multicolumn{2}{c}{Natural Ques.} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14}
 & & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) \\
\midrule
\multirow{4}{*}{V 7B}
 & Medusa & 1.91x & 2.52 & 2.02x & 2.67 & 1.89x & 2.59 & 1.79x & 2.48 & 1.42x & 2.02 & 1.51x & 2.09 \\
 & EAGLE & 2.90x & 3.94 & 3.33x & 4.29 & 3.01x & 4.00 & 2.79x & 3.89 & 2.33x & 3.42 & 2.31x & 3.21 \\
 & EAGLE-2 & 3.62x & 4.98 & 3.95x & 5.33 & 3.63x & 4.97 & 3.46x & 4.86 & 2.94x & 4.12 & 2.76x & 3.82 \\
 & ReDrafter & 2.78x & 4.12 & 2.73x & 4.14 & 2.65x & 3.84 & 2.89x & 4.18 & 1.98x & 3.07 & 2.00x & 3.07 \\
\bottomrule
\multirow{4}{*}{V 13B}
 & Medusa & 2.07x & 2.59 & 2.50x & 2.78 & 2.23x & 2.64 & 2.08x & 2.45 & 1.71x & 2.09 & 1.81x & 2.10 \\
 & EAGLE & 3.07x & 3.98 & 3.58x & 4.39 & 3.08x & 3.97 & 3.03x & 3.95 & 2.49x & 3.52 & 2.42x & 3.11\\
 & EAGLE-2 & 4.26x & 4.83 & 4.96x & 5.41 & 4.22x & 4.79 & 4.25x & 4.89 & 3.40x & 4.21 & 3.13x & 3.74\\
 & ReDrafter & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} \\
\bottomrule
\multirow{4}{*}{V 33B}
 & Medusa & \tbd{2.07x} & \tbd{2.59} & \tbd{2.50x} & \tbd{2.78} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} \\
 & EAGLE & \tbd{3.07x} & \tbd{3.98} & \tbd{3.58x} & \tbd{4.39} & \tbd{3.08x} & \tbd{3.97} & \tbd{3.03x} & \tbd{3.95} & \tbd{3.08x} & \tbd{3.97} & \tbd{3.03x} & \tbd{3.95} \\
 & EAGLE-2 & \tbd{4.26x} & \tbd{4.83} & \tbd{4.96x} & \tbd{5.41} & \tbd{4.22x} & \tbd{4.79} & \tbd{4.25x} & \tbd{4.89} & \tbd{4.22x} & \tbd{4.79} & \tbd{4.25x} & \tbd{4.89} \\
 & ReDrafter & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} \\
\bottomrule
\end{tabular}
}
\label{table:pytorch_benchmark_t0}
\end{table}

==> ICLR2025_submission/tables/pytorch_benchmark_t1.tex <==
\begin{table}[t]
\centering
\caption{Comparison of Speedup and \(\tau\) for Different Methods on Various Benchmarks (t=1). \aonan{Need to mention drafter size.}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
 & & \multicolumn{12}{c}{Benchmark} \\
\cmidrule(l){3-14}
Model & Method & \multicolumn{2}{c}{MT-bench} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{Alpaca} & \multicolumn{2}{c}{CNN/DM} & \multicolumn{2}{c}{Natural Ques.} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14}
 & & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) \\
\midrule
\multirow{4}{*}{V 7B}
 & Medusa & \tbd{2.07x} & \tbd{2.59} & \tbd{2.50x} & \tbd{2.78} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} \\
 & EAGLE & 2.13x & 3.17 & 2.39x & 3.43 & 2.34x & 3.29 & 2.21x & 3.30 & 2.08x & 3.12 & 1.95x & 2.86 \\
 & EAGLE-2 & 3.05x & 4.28 & 3.33x & 4.65 & 3.07x & 4.49 & 3.08x & 4.43 & 2.63x & 3.76 & 2.48x & 3.56 \\
 & ReDrafter & \bf{3.53x} & \bf{5.34} & \bf{3.47x} & \bf{5.31} & \bf{3.28x} & \bf{4.91} & \bf{3.69x} & \bf{5.51} & \bf{2.91x} & \bf{4.54} & \bf{3.04x} & \bf{4.59} \\
\bottomrule
\multirow{4}{*}{V 13B}
 & Medusa & \tbd{2.07x} & \tbd{2.59} & \tbd{2.50x} & \tbd{2.78} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} \\
 & EAGLE & 2.32x & 3.20 & 2.65x & 3.63 & 2.57x & 3.60 & 2.45x & 3.57 & 2.23x & 3.26 & 2.14x & 3.06 \\
 & EAGLE-2 & 3.80x & 4.40 & 4.22x & 4.89 & 3.77x & 4.41 & 3.78x & 4.37 & 3.25x & 3.97 & 3.07x & 3.54 \\
 & ReDrafter & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} \\
\bottomrule
\multirow{4}{*}{V 33B}
 & Medusa & \tbd{2.07x} & \tbd{2.59} & \tbd{2.50x} & \tbd{2.78} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} & \tbd{2.23x} & \tbd{2.64} & \tbd{2.08x} & \tbd{2.45} \\
 & EAGLE & \tbd{3.07x} & \tbd{3.98} & \tbd{3.58x} & \tbd{4.39} & \tbd{3.08x} & \tbd{3.97} & \tbd{3.03x} & \tbd{3.95} & \tbd{3.08x} & \tbd{3.97} & \tbd{3.03x} & \tbd{3.95} \\
 & EAGLE-2 & \tbd{4.26x} & \tbd{4.83} & \tbd{4.96x} & \tbd{5.41} & \tbd{4.22x} & \tbd{4.79} & \tbd{4.25x} & \tbd{4.89} & \tbd{4.22x} & \tbd{4.79} & \tbd{4.25x} & \tbd{4.89} \\
 & ReDrafter & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} & \tbd{5.00x} & \tbd{6.00} \\
\bottomrule
\end{tabular}
}
\label{table:pytorch_benchmark_t1}
\end{table}

==> ICLR2025_submission/tables/pytorch_benchmark_v3.tex <==
\begin{table}[t]
\centering
\caption{Speedup and Tokens/Step on MT-Bench and AlpacaEval.}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{7}{c}{MT-bench,~temperature=0} \\
\toprule
\multirow{2}{*}{Method} 
%& \multirow{2}{*}{Category} 
& \multicolumn{2}{c}{Vicuna 7B} & \multicolumn{2}{c}{Vicuna 13B} & \multicolumn{2}{c}{Vicuna 33B} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
% \cmidrule(l){7-8} 
& Speedup & Tokens/Step & Speedup & Tokens/Step & Speedup & Tokens/Step  \\
% \midrule
% \multirow{8}{*}{ReDrafter} 
% & Writing & 2.77x & 4.18 & 2.70x & 4.00 & 2.50x & 3.63 \\
% & Roleplay & 2.91x & 4.50 & 2.80x & 4.22 & 2.47x & 3.64 \\
% & Reasoning & 2.59x & 3.85 & 2.60x & 3.87 & 2.68x & 3.73 \\
% & Math & 2.96x & 4.34 & 3.11x & 4.61 & 3.26x & 4.32 \\
% & Coding & 3.19x & 4.86 & 3.21x & 4.88 & 3.26x & 4.49 \\
% & Extraction & 2.91x & 4.39 & 3.08x & 4.59 & 3.12x & 4.32 \\
% & Stem & 2.80x & 4.28 & 2.74x & 4.28 & 2.61x & 3.79 \\
% & Humanities & 2.52x & 3.69 & 2.69x & 3.92 & 2.47x & 3.43 \\
\midrule
Medusa & 2.39x & 2.55 & 2.40x & 2.61 & 2.51x & 2.53\\
EAGLE & 2.69x & 3.96 & 2.74x & 4.00 & \bf{2.80x} & 3.71\\
ReDrafter & \bf{2.80x} & \bf{4.20} & \bf{2.80x} & \bf{4.21} & 2.61x & \bf{3.87} \\
\midrule
\multicolumn{7}{c}{MT-bench,~temperature=1} \\
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Vicuna 7B} & \multicolumn{2}{c}{Vicuna 13B} & \multicolumn{2}{c}{Vicuna 33B} \\
% \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} 
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
 & Speedup & Tokens/Step & Speedup & Tokens/Step & Speedup & Tokens/Step  \\
% \midrule
% \multirow{8}{*}{ReDrafter} 
% & Writing & 3.58x & 5.52 & 3.46x & 5.44 & 3.24x & 4.69\\
% & Roleplay & 3.59x & 5.54 & 3.66x & 5.45 & 3.39x & 4.95 \\
% & Reasoning & 3.47x & 5.29 & 3.25x & 5.13 & 3.12x & 4.42 \\
% & Math & 3.63x & 5.43 & 3.56x & 5.13 & 3.37x & 4.83\\
% & Coding & 3.75x & 5.57 & 3.70x & 5.56 & 3.58x & 5.05 \\
% & Extraction & 3.16x & 4.85 & 3.29x & 5.01 & 2.94x & 4.34 \\
% & Stem & 3.32x & 5.00 & 3.69x & 5.40 & 3.35x & 4.75 \\
% & Humanities & 3.49x & 5.27 & 3.46x & 5.17 & 3.13x & 4.52 \\
\midrule
Medusa & 2.33x &2.55 & 2.36x & 2.61 & 2.52x & 2.59 \\
EAGLE & 2.31x & 3.51 & 2.27x & 3.55 & 2.63x & 3.48 \\
ReDrafter & \bf{3.50x} & \bf{5.31} & \bf{3.51x} & \bf{5.29} & \bf{3.27x} & \bf{4.69} \\
\midrule
\multicolumn{7}{c}{AlpacaEval,~temperature=0} \\
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{2}{c}{Vicuna 7B} & \multicolumn{2}{c}{Vicuna 13B} & \multicolumn{2}{c}{Vicuna 33B} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
% \cmidrule(l){7-8} 
& Speedup & Tokens/Step & Speedup & Tokens/Step & Speedup & Tokens/Step  \\
\midrule
Medusa & 2.19x & 2.42 & 2.26x & 2.45 & 2.31x & 2.31\\
EAGLE & 2.43x & 3.61 & 2.49x & 3.62 & \bf{2.59x} & 3.29 \\
ReDrafter & \bf{2.69x} & \bf{4.06} & \bf{2.78x} & \bf{4.02} & 2.43x & \bf{3.61} \\
\midrule
\multicolumn{7}{c}{AlpacaEval,~temperature=1} \\
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Vicuna 7B} & \multicolumn{2}{c}{Vicuna 13B} & \multicolumn{2}{c}{Vicuna 33B} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
 & Speedup & Tokens/Step & Speedup & Tokens/Step & Speedup & Tokens/Step  \\
\midrule
Medusa & 2.26x & 2.42 & 2.24x & 2.50 & 2.34x & 2.43 \\
EAGLE &  2.20x & 3.29 & 2.16x & 3.34 & 2.41x & 3.16 \\
ReDrafter & \bf{3.53x} & \bf{5.31} & \bf{3.50x} & \bf{5.22} & \bf{3.32x} & \bf{4.71} \\
\bottomrule
\end{tabular}
}
\label{table:pytorch_benchmark_v2}
\end{table}
% \begin{table}[t]
% \centering
% \caption{Speedup and \(\tau\) for Medusa, EAGLE, and ReDrafter on MT-Bench.}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lccccccccccccccccccccc@{}}
% \toprule
% \multicolumn{18}{c}{MT-bench,~temperature=0 \cmnt{7B 33.43, 13B 26.89, 33B 16.61}} \\
% \toprule
% \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Writing} & \multicolumn{2}{c}{Roleplay} & \multicolumn{2}{c}{Reasoning} & \multicolumn{2}{c}{Math} & \multicolumn{2}{c}{Coding} & \multicolumn{2}{c}{Extraction} & \multicolumn{2}{c}{Stem} & \multicolumn{2}{c}{Humanities} & \multicolumn{2}{c}{Average} \\
% \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14} \cmidrule(l){15-16} \cmidrule(l){17-18} \cmidrule(l){19-20} \cmidrule(l){21-22}
%  & & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) & Speedup & \(\tau\) \\
% \midrule
% \multirow{3}{*}{V 7B}
%  & Medusa & 2.27x\cmnt{76.11} & 2.41 & 2.26x\cmnt{75.69} & 2.41 & 2.27x\cmnt{76.03} & 2.47 & 2.57x\cmnt{85.98} & 2.75 & 2.71x\cmnt{90.66} & 2.86 & 2.55x\cmnt{85.35} & 2.74 & 2.34x\cmnt{78.49} & 2.48 & 2.17x\cmnt{72.67} & 2.29 & 2.39x & 2.55 \\
%  & EAGLE & 2.47x\cmnt{82.68} & 3.56 & 2.61x\cmnt{87.54} & 3.83 & 2.54x\cmnt{84.98} & 3.81 & 2.89x\cmnt{96.70} & 4.24 & 3.11x\cmnt{104.30} & 4.58 & \bf{2.91x}\cmnt{97.32} & \bf{4.39} & 2.54x\cmnt{85.03} & 3.71 & 2.45x\cmnt{82.17} & 3.52 & 2.69x & 3.96 \\
%  & ReDrafter & \bf{2.77x} & \bf{4.18} & \bf{2.91x} & \bf{4.50} & \bf{2.59x} & \bf{3.85} & \bf{2.96x} & \bf{4.34} & \bf{3.19x} & \bf{4.86} & {2.62x} & {3.93} & \bf{2.80x} & \bf{4.28} & \bf{2.52x} & \bf{3.69} & \bf{2.80x} & \bf{4.20}\\
% \midrule
% \multirow{3}{*}{V 13B}
%  & Medusa & 2.27x\cmnt{61.10} & 2.46 & 2.28x\cmnt{61.37} & 2.48 & 2.21x\cmnt{59.46} & 2.46 & 2.66x\cmnt{71.71} & 2.89 & 2.75x\cmnt{73.97} & 2.97 & 2.43x\cmnt{65.45} & 2.66 & 2.36x\cmnt{63.48} & 2.54 & 2.23x\cmnt{60.02} & 2.39 & 2.40x & 2.61 \\
%  & EAGLE & 2.59x\cmnt{69.82} & 3.74 & 2.41x\cmnt{64.92} & 3.48 & 2.51x\cmnt{67.64} & 3.80 & 3.08x\cmnt{82.99} & 4.49 & 3.07x\cmnt{82.79} & 4.43 & \bf{3.08x}\cmnt{82.88} & \bf{4.59} & 2.64x\cmnt{71.15} & 3.81 & 2.53x\cmnt{68.25} & 3.65 & 2.74x & 4.00 \\
%  & ReDrafter & \bf{2.70x} & \bf{4.00} & \bf{2.80x} & \bf{4.22} & \bf{2.60x} & \bf{3.87} & \bf{3.11x} & \bf{4.61} & \bf{3.21x} & \bf{4.88} & {2.52x} & {3.91} & \bf{2.74x} & \bf{4.28} & \bf{2.69x} & \bf{3.92} & \bf{2.80x} &\bf{4.21} \\
% \midrule
% \multirow{3}{*}{V 33B}
%  & Medusa & 2.24x\cmnt{37.37} & 2.24 & 2.33x\cmnt{38.86} & 2.32 & 2.44x\cmnt{40.60} & 2.48 & 2.83x\cmnt{47.15} & 2.82 & 2.90x\cmnt{48.20} & 2.94 & 2.71x\cmnt{45.09} & 2.85 & 2.40x\cmnt{40.01} & 2.40 & 2.25x\cmnt{37.43} & 2.22 & 2.51x & 2.53\\
%  & EAGLE & 2.47x\cmnt{41.15} & 3.23 & 2.42x\cmnt{40.36} & 3.17 & \bf{2.68x}\cmnt{44.54} & 3.63 & \bf{3.26x}\cmnt{54.24} & 4.30 & \bf{3.36x}\cmnt{55.87} & 4.41 & \bf{3.12x}\cmnt{51.90} & \bf{4.32} & \bf{2.61x}\cmnt{43.49} & 3.41 & \bf{2.47x}\cmnt{41.06} & 3.21 & \bf{2.80x} & 3.71 \\
%  & ReDrafter & \bf{2.50x} & \bf{3.63} & \bf{2.47x} & \bf{3.64} & {2.47x} & \bf{3.73} & {2.72x} & \bf{4.32} & {3.25x} & \bf{4.49} & {2.62x} & {3.95} & {2.55x} & \bf{3.79} & {2.26x} & \bf{3.43} & {2.61x} & \bf{3.87} \\
% \midrule
% \multicolumn{18}{c}{MT-bench,~temperature=1 \cmnt{7B 32.14, 13B 26.88, 33B 15.88}} \\
% \toprule
% \multirow{3}{*}{V 7B}
%  & Medusa & 2.09x\cmnt{67.48} & 2.28 & 2.24x\cmnt{72.24} & 2.46 & 2.23x\cmnt{71.78} & 2.52 & 2.52x\cmnt{81.18} & 2.77 & 2.57x\cmnt{82.71} & 2.78 & 2.45x\cmnt{78.83} & 2.70 & 2.31x\cmnt{74.51} & 2.52 & 2.21x\cmnt{71.13} & 2.39 & 2.33x & 2.55 \\
%  & EAGLE & 2.21x\cmnt{69.39} & 3.23 & 2.12x\cmnt{68.27} & 3.20 & 2.17x\cmnt{69.95} & 3.50 & 2.50x\cmnt{80.46} & 3.83 & 2.67x\cmnt{85.85} & 4.00 & 2.46x\cmnt{79.31} & 3.79 & 2.21x\cmnt{71.30} & 3.32 & 2.14x\cmnt{69.08} & 3.20 & 2.31x & 3.51 \\
%  & ReDrafter & \bf{3.58x} & \bf{5.52} & \bf{3.59x} & \bf{5.54} & \bf{3.47x} & \bf{5.29} & \bf{3.63x} & \bf{5.43} & \bf{3.75x} & \bf{5.57} & \bf{3.16x} & \bf{4.85} & \bf{3.32x} & \bf{5.00} & \bf{3.49x} & \bf{5.27} & \bf{3.50x} & \bf{5.31} \\
% \midrule
% \multirow{3}{*}{V 13B}
%  & Medusa & 2.22x\cmnt{59.90} & 2.47 & 2.22x\cmnt{59.90} & 2.47 & 2.23x\cmnt{59.98} & 2.53 & 2.60x\cmnt{69.98} & 2.91 & 2.64x\cmnt{71.05} & 2.92 & 2.40x\cmnt{64.67} & 2.69 & 2.35x\cmnt{63.30} & 2.54 & 2.21x\cmnt{59.45} & 2.38  & 2.36x & 2.61 \\`
%  & EAGLE & 1.98x\cmnt{53.24} & 3.05 & 2.11x\cmnt{56.86} & 3.27 & 2.22x\cmnt{59.70} & 3.57 & 2.45x\cmnt{65.99} & 3.83 & 2.58x\cmnt{69.54} & 3.99 & 2.40x\cmnt{64.78} & 3.83 & 2.28x\cmnt{61.43} & 3.54 & 2.12x\cmnt{57.24} & 3.30 & 2.27x & 3.55 \\
%  & ReDrafter & \bf{3.46x} & \bf{5.44} 
%             & \bf{3.66x} & \bf{5.45} 
%             & \bf{3.25x} & \bf{5.13} 
%             & \bf{3.56x} & \bf{5.13} 
%             & \bf{3.70x} & \bf{5.56} 
%             & \bf{3.29x} & \bf{5.01} 
%             & \bf{3.69x} & \bf{5.40} 
%             & \bf{3.46x} & \bf{5.17} 
%             & \bf{3.51x} & \bf{5.29}\\
% \midrule
% \multirow{3}{*}{V 33B}
%  & Medusa & 2.28x\cmnt{36.25} & 2.19 & 2.50x\cmnt{39.74} & 2.37 & 2.55x\cmnt{40.51} & 2.46 & 2.90x\cmnt{46.21} & 2.75 & 3.03x\cmnt{48.21} & 2.97 & 2.72x\cmnt{43.31} & 2.79 & 2.46x\cmnt{39.14} & 2.40 & 2.28x\cmnt{36.34} & 2.23 & 2.59x & 2.52 \\
%  & EAGLE & 2.22x\cmnt{35.33} & 2.93 & 2.38x\cmnt{37.92} & 3.14 & 2.57x\cmnt{40.93} & 3.47 & 2.98x\cmnt{47.43} & 3.89 & 3.18x\cmnt{50.64} & 4.14 & 2.84x\cmnt{45.16} & 3.91 & 2.45x\cmnt{38.98} & 3.18 & 2.41x\cmnt{38.37} & 3.14 & 2.63x & 3.48\\
%  & ReDrafter & \bf{3.24x} & \bf{4.69} 
%             & \bf{3.39x} & \bf{4.95} 
%             & \bf{3.12x} & \bf{4.42} 
%             & \bf{3.37x} & \bf{4.83} 
%             & \bf{3.58x} & \bf{5.05} 
%             & \bf{2.94x} & \bf{4.34} 
%             & \bf{3.35x} & \bf{4.75} 
%             & \bf{3.13x} & \bf{4.52} 
%             & \bf{3.27x} & \bf{4.69}\\
% \bottomrule
% \end{tabular}
% }
% \label{table:pytorch_benchmark_mt_bench_v2}
% \end{table}

% % TODO add a highlight to rows of ReDrafter
% % TODO consider another presentation to distinguash from Eagle, or Change the table to bar plots? Or Transpose?


==> ICLR2025_submission/tables/trt_experiments.tex <==
% \begin{table}[t]
% \centering
% \caption{TensorRT-LLM experiments on MT-bench: (left) offline mode with varying tensor parallelism, and (right) continuous batching mode with different request rates.}
% \resizebox{.95\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccc|cccccccccc@{}}
% \toprule
%  & \multicolumn{6}{c|}{Offline TensorRT-LLM (Tensor Parallelism)} & \multicolumn{6}{c}{Continuous Batching TensorRT-LLM (Request Rate QPS)} \\
% \cmidrule(l){2-13}
% Model & \multicolumn{2}{c}{Tensor Parallelism=1} & \multicolumn{2}{c}{Tensor Parallelism=2} & \multicolumn{2}{c|}{Tensor Parallelism=4} & \multicolumn{2}{c}{QPS=0.1} & \multicolumn{2}{c}{QPS=0.5} & \multicolumn{2}{c}{QPS=1.0} \\
% \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} \cmidrule(l){12-13}
%  & TPS & Speedup & TPS & Speedup & TPS & Speedup & ms/token & Speedup & ms/token & Speedup & ms/token & Speedup \\
% \midrule
% V 7B & 323.12 & 2.19x & 373.27 & 1.82x & 403.87 & 1.68x & 2.41 & 2.09x & 2.48 & 2.11x & 2.76 & 1.57x \\
% V 13B & 198.64 & 2.30x & 251.55 & 1.89x & 312.79 & 1.84x & 3.41 & 2.31x & 3.61 & 1.71x & 5.43 & 1.22x \\
% V 33B & 97.5 & 2.51x & 137.47 & 2.15x & 171.11 & 1.93x & 5.93 & 2.56x & 9.85 & 1.27x & \tbd{100.0} & \tbd{5.00} \\
% \bottomrule
% \end{tabular}
% }
% \label{table:trt_experiments}
% \end{table}

\begin{table}[t]
\centering
\caption{ TensorRT-LLM experiments on MT-bench with continuous batching at varying request rates, using fixed settings of TP=1, beam width=6, beam length=5, and temperature=1.}
% Tensor Parallelism of LLM is 1. Beam width is 6, and beam length is 5.
% \tbd{bw6 x bl5}
\resizebox{.7\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 % & \multicolumn{6}{c}{Continuous Batching TensorRT-LLM (Request Rate QPS)} \\
 & \multicolumn{6}{c}{Request Rate Queries Per Second (QPS)} \\
\cmidrule(l){2-7}
Model & \multicolumn{2}{c}{QPS=0.1} & \multicolumn{2}{c}{QPS=0.5} & \multicolumn{2}{c}{QPS=1.0} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
 & ms/token & Speedup & ms/token & Speedup & ms/token & Speedup \\
\midrule
V 7B & 2.41 & 2.09x & 2.48 & 2.11x & 2.76 & 1.57x \\
V 13B & 3.41 & 2.31x & 3.61 & 1.71x & 5.43 & 1.22x \\
V 33B & 5.93 & 2.56x & 8.41 & 1.49x & 20.04 & 1.37x \\
\bottomrule
\end{tabular}
}
\label{table:trt_experiments_qps}
\end{table}

\begin{table}[t]
\centering
% \caption{\tbd{Offline / Static Batching} TensorRT-LLM experiments on MT-bench with varying tensor parallelism. Batch size is 1.}
\caption{TensorRT-LLM experiments on MT-bench using static batching with varying tensor parallelism (TP). We fix batch size=1, beam width=6, beam length=5, and temperature=1.}
\resizebox{.7\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 % & \multicolumn{6}{c}{Offline TensorRT-LLM (Tensor Parallelism)} \\
 & \multicolumn{6}{c}{\# Tensor Parallelism (TP) of LLM} \\
\cmidrule(l){2-7}
Model & \multicolumn{2}{c}{TP=1} & \multicolumn{2}{c}{TP=2} & \multicolumn{2}{c}{TP=4} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
 & TPS & Speedup & TPS & Speedup & TPS & Speedup \\
\midrule
V 7B & 323.12 & 2.19x & 373.27 & 1.82x & 403.87 & 1.68x \\
V 13B & 198.64 & 2.30x & 251.55 & 1.89x & 312.79 & 1.84x \\
V 33B & 97.50 & 2.51x & 137.47 & 2.15x & 171.11 & 1.93x \\
\bottomrule
\end{tabular}
}
\label{table:trt_experiments_tp}
\end{table}

